Capacitated Team Formation Problem on Social Networks

In a team formation problem, one is required to find a group of users that can match the requirements of a collaborative task. Example of such collaborative tasks abound, ranging from software product development to various participatory sensing tasks in knowledge creation. Due to the nature of the task, team members are often required to work on a co-operative basis. Previous studies have indicated that co-operation becomes effective in presence of social connections. Therefore, effective team selection requires the team members to be socially close as well as a division of the task among team members so that no user is overloaded by the assignment. In this work, we investigate how such teams can be formed on a social network. Since our team formation problems are proven to be NP-hard, we design efficient approximate algorithms for finding near optimum teams with provable guarantees. As traditional data-sets from on-line social networks (e.g. Twitter, Facebook etc) typically do not contain instances of large scale collaboration, we have crawled millions of software repositories spanning a period of four years and hundreds of thousands of developers from GitHub, a popular open-source social coding network. We perform large scale experiments on this data-set to evaluate the accuracy and efficiency of our algorithms. Experimental results suggest that our algorithms achieve significant improvement in finding effective teams, as compared to naive strategies and scale well with the size of the data. Finally, we provide a validation of our techniques by comparing with existing software teams in GitHub.

==> concl.tex <==
\section{Conclusion}
%\vspace{-.1in}
\label{sec:concl}
In this work, we presented a novel team-formation problem on social networks
that attempts to find teams that are socially close as well as division of the
task so that no user is overloaded by the assignment.
%We observe that parallel to reducing the collaboration cost, the issue of 
%obeying the capacity constraints of the users plays a key role in determining 
%the best team. 
We presented algorithms for this problem under different models of social collaboration and
analyzed their performance thoroughly. Our experiments with real-life data-sets show that
these techniques outperform the naive strategies by a significant margin.
$\\$


==> exten.tex <==
\section{Extensions}
\label{sec:extn}

In this section, we describe some key extensions of our problem
and briefly outline how our algorithms can be modified to handle those cases.
%. For sake of brevity,
%we will restrict ourselves to the uniform model of capacities.

\par{{\bf Price on users:}} In a real-world situation, users are often paid
for their participation in a task. In such a scenario, 
the objective of the team formation problem is not only to 
find teams that
minimize the
social collaboration cost but also to account for the price paid to the 
users. One approach could be to define the cost of a team of users $U$ in the following
way: $\alpha\sum_{u\in U}\pi_u + \beta f(U)$, where $\pi_u$ is the price
paid to user $u \in U$ and $f(\cdot)$ represents the social 
collaboration cost (see Section~\ref{subsec:costmodels}). Here $\alpha,\beta >0$
are parameters to the problem. The objective is to find the team with least
total cost.

In order to account for the modified cost function, we pre-process the social
networking graph in the following way. For each user $u$, create a new node $u'$
and add an edge $(u,u')$ with the cost $\alpha\cdot \pi_u$ i.e. $w(u,u')=\alpha\cdot \pi_u$.
In the next step, multiply each edge cost in the original graph by a factor $\beta$ i.e.
the cost of the edge $(u,v)$ is set to $\beta\cdot w(u,v)$. Finally, we make the following
sequence of assignments: $I_{u'} \leftarrow I_u,c_{u'} \leftarrow c_u,I_u = 0, c_u = 0$.
With this pre-processing in place, we can use the algorithms \diamsol\ and \steinersol\ on the
modified graph to 
compute the approximate solutions and the approximation factors remain unchanged. 
%It can be shown that the approximation factors for
%these algorithms remain unchanged. 

\par{{\bf Multiple units of items:}} We consider another generalization where a task
is a multi-set of items of the form $T=\{(i_1,n_1),(i_2,n_2),\cdots,(i_k,n_k)\}$
where $\{i_1,i_2,\cdots,i_k\}$ are the set of items needed for the task and $n_j$ is
the multiplicity of item $i_j$ i.e. the number of units required for item $i_j$.
In this setting, a user $u$ can be assigned zero or more units of item $i$ if $i\in I_u$
and the total unit of all the items assigned to $u$ can be no more than her capacity.

We first modify Lemma~\ref{lem:feasibility} to account for the multiplicities of items.
In the construction of the flow network, we set the capacities of the edges of the 
form $(l_i,r_u)$ to $n_i$, where $i$ is an item in the task and $u$ is a user. Moreover,
edges of the form $(s,l_i)$ have capacities $n_i$. It can be verified that if the maximum
flow has value $\sum_{i\in T} n_i$ then there is a feasible team. 
%Otherwise, the flow value
%corresponds to the maximum total units of items that can be allocated to a given team of users.
With this modification of the \maxcover\ procedure, we can apply algorithms \diamsol\ and \steinersol\ 
to obtain the approximate teams. 
It can be shown that while the \diamsol\ algorithm achieves a factor of $2$
approximation, the \steinersol\ algorithm has an approximation ratio of $O(\log k \sum_{i\in T}n_i)$. 
%We leave
%the improvement of approximation ratio for \steinersol\, as a future work. 


==> optimization.tex <==
\section{Optimizations}
\label{sec:opt}

In this section, we present some optimization techniques to
speed up our team formation algorithms. 

\subsection{Clustering}

\subsection{Distance Oracle}




==> related.tex <==
\section{Related Work}
%\vspace{-.05in}
\label{sec:related}

Team formation is a well-studied problem 
in the Operations Research (OR)
community~\cite{Baykasoglu2007,Wi2009,Zzkarian1999,Abdelsalam2009}.
In their setting, the goal is to find an allocation of tasks
to different individuals so as to satisfy the project requirements.
%The trend in this body of work is to model it as an optimization
%problem to find the best match between people and the functional
%requirements of a project. 
However, this body of work ignores the 
social relationship among people while deciding the best team and unfortunately,
their techniques can not be applied to solve our problem.

Lappas et.al~\cite{Lappas2009} considered the problem of 
finding team of experts on a social
network. 
%According to their model, the professionals or skilled individuals are
%organized on a social network to represent their collaboration costs. 
Given a requirement of skills, their goal is to find a team that 
minimizes the overall communication cost. Although they have a similar
objective in mind, our problem is fundamentally very different from them.
In~\cite{Lappas2009}, the authors don't deal with capacities on users. 
In effect, their problem can be
thought of as {\it uncapacitated} version of our problem. As per our
understanding, the notion of capacity changes the problem structure completely
and their solutions can no longer be adapted to handle our requirement. Moreover,
through detailed experiments (see Section~\ref{sec:expts}), we have 
established that a natural extension of
their algorithms perform very poorly compared to ours.

In~\cite{Anagnostopoulos2010}, the authors studied a version of the team formation 
problem where the goal was to balance the load (\ie the number of projects one is 
assigned to) of individuals. However, this version of the problem overlooks the social collaboration 
cost altogether. In a more recent study~\cite{Anagnostopoulos2012}, the authors present algorithms which, 
in addition to load balance, also find teams with bounded social collaboration cost. Their formulation 
is, however, different from ours - in addition to finding teams with bounded collaboration cost,
they attempt to minimize the load on team members, whereas, we take the user capacities as constraint
and attempt to minimize the social collaboration cost.
%complimentary to our formulation in finding teams that satisfy capacity constraints on users 
%and minimize the collaboration
%cost whereas, their formulation takes the collaboration cost as a constraint, attempt to minimize the
%load on users.
%
%In our formulation, capacities are hard constraints and the algorithms are designed to satisfy them
%for each individuals.  
%
% In that spirit, their problem is formulated as a soft constraint on capacities
%and does not
%Although their notion 
%of social collaboration cost is similar to ours in spirit, none of the notions of load 
%balancing they study 
%preclude the possibility of overloading certain individuals.


%The paper closely related to our work is by Lappas et.al~\cite{Lappas2009}.
%In~\cite{Lappas2009}, the authors 
%assume that people communicate through their
%social links and communication through these links incur cost that depend
%on several factors like relationship strengths etc. 
%Therefore the best team will naturally correspond to the one leading to
%the least communication cost. However, the crucial difference from our work is that
%they assume people having infinite capacity and whenever selected, a person
%can apply all of her skills simultaneously. This is in stark contrast with reality;
%in practice, people are limited by their capacity which primarily depends on the
%amount of time they can spend on a task in a daily basis.
%, but not limited to exclude other
%factors like availability of computing resources, network bandwith etc. 
%This changes
%the problem structure significantly and makes our problem non-trivial to approximate using 
%known techniques. 
%It is important to point out that the algorithms presented in~\cite{Lappas2009}
%can not be adapted in a straightforward way to accommodate the capacities.

%Another related body of work is the research on the Group Steiner Tree (GST) 
%problem~\cite{Garg2000,Even2002}. However, unlike in our setting, GST does
%not have the notion of capacities. Therefore, the algorithms and techniques presented
%there can not be used directly in our case. It is possible to adapt the 
%rounding technique outlined in~\cite{Garg2000} to yield an algorithm that finds
%an O($\log ^3n \log k$) factor approximate solution with a blow-up of the capacities by a 
%factor of O($\log n \cdot \log k$). Moreover, it can be proved that
%such a blow-up of capacities is essential to bound the approximation factor.
%\footnote{We will include the details of the algorithm and
%proof in the full version of the paper.} However, we believe 
%that such an algorithm is not practical
%for a couple of reasons. For a large social network having millions of users, 
%O($\log^3 n$) is a prohibitively large number to appear in the approximation factor
%(e.g. Facebook with nearly 500 million users, $\log^3 n \approx 650$). Moreover, severe 
%blow-up
%of capacities may not be acceptable in real-life applications.(e.g. forming a team of
%developers for projects). Therefore, we will treat capacities as hard constraints and 
%design algorithms where all these constraints are absolutely satisfied.

%A more closely related work, on a theoretical
%front, is by Chuzoy et al~\cite{Chuzhoy2002}, where they present approximation algorithms
%for capacitated covering problems. Unfortunately, their algorithms cater to only a specific
%instance of our problem and therefore, we can not borrow their techniques to apply to
%our problem in its
%for the capacitated set
%cover problem can not be applied directly to our problem in its 
%full generality~\footnote{Please
%see Section~\ref{sec:capset} for a detailed comparison.}.
%where they consider the social connections among the individuals in the form
%of communication cost and formulate the team formation problem to minimize
%this cost. 

The specific techniques required to estimate the strength of relationship among
individuals is an active and important area of research that has been pursued in
other research works~\cite{Xiang2010, Leskovec2010}. However, we believe that
this direction of research is orthogonal and beyond the scope and goal of this paper.

